Advancing Experimental Platforms for UAV Communications: Insights from AERPAW'S Digital Twin

The rapid evolution of 5G and beyond has advanced space-air-terrestrial networks, with unmanned aerial vehicles (UAVs) offering enhanced coverage, flexible configurations, and cost efficiency. However, deploying UAV-based systems presents challenges including varying propagation conditions and hardware limitations. While simulators and theoretical models have been developed, real-world experimentation is critically important to validate the research. Digital twins, virtual replicas of physical systems, enable emulation that bridge theory and practice. This paper presents our experimental results from AERPAW's digital twin, showcasing its ability to simulate UAV communication scenarios and providing insights into system performance and reliability.

==> Tables/ORANusecasesTable.tex <==
\begin{table*}[ht]
\centering
\caption{Representative O-RAN use cases employing AI \textcolor{black}{as defined by the O-RAN Alliance~\cite{li2020ran}}. %\hl{Add a few xApp use case that have demonstrated O-RAN.}
}
\footnotesize
%\resizebox{0.85\textwidth}{!}{%
%\begin{tabular}{|c|c|c|c|}
{\begin{tabular}{|p{1.7cm}|p{0.9cm}|p{3.5cm}|p{0.9cm}|p{1cm}|p{4.4cm}|p{2.7cm}|}
\hline
 \textbf{Use case} &\textbf{Network layer} &  \textbf{AI %models
 functionality description}  &   \textbf{Training host}  & \textbf{Inference host }  &   \textbf{Training data}  &  \textbf{Action} 

\\ \hline
%\vspace{0.001 in} 
Massive MIMO beamforming optimization 
& PHY  
& Predict the optimal configuration of massive MIMO parameters for each cell according to a global optimization objective designed by the operator. 
&  Non-RT RIC &  Non-RT RIC 
& Key performance indicators (KPIs) related to traffic load, coverage and QoS performance, per beam/area and massive MIMO configuration.
& Configure the optimized beam parameters via the O1 interface.
\\ \hline

%\vspace{0.001 in}
Quality of experience (QoE) optimization 
& MAC  
& %Making predictions on
Predict the application/traffic types, QoE and available bandwidth. 
& Non-RT RIC 
& Near-RT RIC 
& Network level measurement report including UE data, L2 measurement, RAN protocol stack status, cell level information, QoE measurement metrics and user traffic. 
& E2 control or policy commands towards the RAN for the QoE optimization.
\\ \hline

%\vspace{0.001 in} 
Dynamic spectrum sharing (DSS) 
& MAC  
& Predict the short-term traffic demand %for 4G and 5G network 
based on near-RT metrics from the RAN. 
& Non-RT RIC  
& Near-RT RIC 
& Location, DSS modality, cell configuration, used, reserved, requested, and blocked PHY resource blocks (PRBs), number of active UEs, traffic demand, QoS classes, and UE capability %and UE location 
information. 
& E2 control/policy of resource configuration and scheduling coordination.
\\ \hline

%\vspace{0.001 in} 
Network slice subnet instance (NSSI) resource allocation optimization 
& MAC  
& Predict of the traffic demand patterns of NSSI at different times and locations. 
& Non-RT RIC & NA 
& Measurement counters per slicing subnet instance. These  include downlink (DL) and uplink (UL) PRBs used for data traffic, average DL and UL throughput, % in gNB average UL UE throughput in gNB, 
and the number of %requested
packet data unit sessions % to setup, Number of PDU sessions 
successfully set up and %number of PDU sessions 
failed to set up.
& Reconfigure the NSSI attributes via the O1 interface and update the Cloud resources via the O2 interface.
\\ \hline
Context-based dynamic handover (HO) management for vehicular users 
& MAC  
& Customize HO sequences for a UE according to intents, policies, and configurations taking into consideration the high speeds and the heterogeneous environment of vehicular UEs.
& Non-RT RIC 
& Near-RT RIC 
& Historic data from %\hl{V2X} 
a vehicular UE over the V1 interface, which include %V2X 
UE location, velocity, and trajectory, %, navigation information. %, \hl{GPS} data. %, CAMs, DENMs. 
measurement reports for serving and neighboring cells, and connection and mobility statistics. 
& RAN deploys the configuration received from the near-RT RIC over the E2 interface.
\\ \hline
%Flight path based dynamic 
Radio resource allocation to unmanned aerial vehicles (UAVs)
& MAC  
& Perform the radio resource allocation %for on-demand coverage 
for UAVs to tackle %introduced 
challenges %as the height increase, 
such as %\hl{LoS} propagation/UL 
RF interference, poor KPIs caused by base station antenna patters (side lobes towards sky). %, and sudden drops in signal strengths.  
& Non-RT RIC 
& Near-RT RIC 
& Aerial vehicle related measurement metrics %from network 
from SMO and based on UE measurement reports, radio channel information, mobility related metrics, flight path, climate, %flight
forbidden/limited 3D area %and space load 
information, etc. %from application, e.g. unmanned aircraft system traffic management. % (UTM). 
& The near-RT RIC delivers the radio resource allocation configurations to the O-CU/O-DU over the E2 interface.
\\ \hline
Traffic steering
& MAC  
& Traffic steering among various RATs, such as LTE, NR, and Wi-Fi, %to enable balanced distribution of traffic 
according to different traffic management    objectives. 
& Non-RT RIC 
& Near-RT RIC 
& Measurement reports, cell load statistics % including intra-RAT and inter-RAT, 
cell quality thresholds, %\hl{CGI}
channel quality indicator reports and measurement gaps on per-UE or per-frequency basis. %Also, cell load statistics including number of active users or connections, number of scheduled users per TTI, and PRB utilization. %, and \hl{CCE} utilization. 
& The traffic management %optimized
policy is activated and transferred to the %E2 nodes 
near-RT RIC via the A1 interface. % to be enforced.
\\ \hline
\end{tabular}%
}

\label{tab:ORANuse}
\end{table*}


==> Tables/ReqTable.tex <==
\begin{table*}
\centering
\caption{Technical Specifications and Design Requirements  Enabling 5G Cellular Networked UAV Research with O-RAN Integration}
\footnotesize
\label{tab:Table_combined}
\begin{tabular}{|p{1.0cm}|p{1.6cm}|p{6.4cm}|p{7.5cm}|}
\hline
\multicolumn{2}{|c|}{\textbf{System Features}} & \textbf{Technical Requirements} & \textbf{Specified Components} \\
\hline
SDR & Data Conversion &
- SDR hardware must support high-resolution ADCs/DACs with sampling rates that can accommodate advanced modulation schemes across a broad RF spectrum. Driver compatibility and community adoption are essential for versatile deployment. &
- USRP B210: ADC Sample Rate (max) 61.44 MS/s, ADC Resolution 12 bits, DAC Sample Rate (max) 61.44 MS/s, DAC Resolution 12 bits, Power Output \textgreater{}10 dBm, ADC Wideband SFDR 78 dBc, Receive Noise Figure \textgreater{}8 dB,  Dimensions 9.7x15.5x1.5 cm, Weight 350 g. \\
\cline{2-4}
& Baseband/ Protocol Processing &
- Requires high-performance multi-core processors capable of handling intensive computational loads, equipped with high-speed data transfer interfaces. &
- Intel NUC13 (mobile node \& fixed node): 6-core i7-10710U, 32 GB RAM, Thunderbolt 3, USB 3.0. \\
\cline{2-4}
& Software &
- Support for advanced network management software, including both open and proprietary solutions, to facilitate a range of experimental configurations. &
- Configurations include USRP Hardware Driver (UHD) v4.3.0, Open Air Interface (OAI) latest branch, open5GS v2.6.4; all hosted on Dockerized Ubuntu 22.04 LTS. Linux   \\
\hline
RF Front End & Amplifier &
- Amplifiers should ensure optimal power output for required coverage while maintaining efficiency to minimize heat generation and power consumption, particularly in mobile setups. &
- Mini-Circuits ZHL-15W-422-S+ for fixed; Mini-Circuits ZVE-8G+ for mobile applications: high gain, efficient power output, suitable for broad operational scenarios. \\
\cline{2-4}
& Filters &
- Must effectively suppress spurious emissions and prevent harmonic interference, configured specifically for the operational frequency bands. &
- Mini-Circuits VLF-4400+ (Tx): Low pass filter, DC-4400 MHz passband. Mini-Circuits VBFZ-3590+ (Rx): Bandpass filter, 3000-4300 MHz operational range. \\
\cline{2-4}
& Antennas &
- Require antennas that offer extensive frequency coverage and adaptability, with considerations for aerodynamic and weight constraints on UAV platforms. &
- Mobile Mark RM-WB1-DN-B1K for fixed; Octane Wireless SA-1400-5900 for mobile nodes: robust coverage, minimal physical footprint. \\
\hline
Network & Experimental Network &
- Must support high-throughput, low-latency connections between RAN and CN, suitable for dynamic and distributed experimental environments. &
- Gigabit Ethernet and WiFi6 (AX4800) ensuring robust, high-speed connectivity suitable for demanding experimental protocols. \\
\cline{2-4}
& Experiment Control &
- Secure and dependable control mechanisms are vital for managing UAVs and network elements remotely under varying experimental conditions. &
- Secured private IP network utilizing SSH protocols over WiFi6, ensuring reliable and secure remote control capabilities. \\
\hline
O-RAN & O-RAN Interface &
- Must support O-RAN Alliance specified open interfaces like E2, A1, and O1/O2, ensuring integration with existing and future RICs and network elements. &
- OAI 5G SA deployment interfaces with the FlexRIC Near RT RIC using an O-RAN complaint E2 interface. \\
\cline{2-4}
& O-RAN RICs &
- Must provide capability for RAN optimizations leveraging O-RAN RICs, supporting AI-driven network management. &
- FlexRIC supports a Near RT RIC terminated by the E2 interface and capable of hosting iApps and xApps. FlexRIC is also capable of integrating with an O-RAN SC RIC.   \\
\cline{2-4}
&  RAN Intelligent Control &
- RIC apps such as xApps and rApps should enable specific optimization and control. &
- KPI Monitor xApp, which provides comprehensive performance metrics for the RAN. Additionally, we utilize a monitoring xApp that gathers metrics from the GTP, MAC, RLC, and PDCP layers, leveraging the KPM SM for enhanced performance monitoring.\\
\cline{2-4}
& O-RAN functional splitting &
- Must provide functional split capabilities that allow for the separation of radio functions between the DU and CU to meet specific deployment needs.  &
- OAI project supports multiple functional splits, including 7.2, 6.2, and 2. We use a traditional deployment of the gnB to support AERPAW's single container E-VM.\\
\cline{2-4}


\hline
\end{tabular}
\end{table*}


==> include/contribution.tex <==
\textcolor{blue}{Extend AI control through the MAC and PHY, from our proposal}
\textcolor{blue}{Describe the architectural changes. and changes proposed in santos.et al (2021) about RANaaS and its security implications}
\textcolor{blue}{Also, explore the integration of transfer learning and architectural changes required for it}

==> include/directions.tex <==
\textcolor{blue}{Can be implicitly described in the previous sections or summarized here}


==> include/resources.tex <==
In this section, we outline the available resources that enable the realization of an open, interoperable and AI driven RAN. %system. 
We first introduce the O-RAN specifications which lays the design foundations and then go on to describe some of the tools and testbeds which have incorporated these principles.

\subsection{Standardization}
\subsubsection{O-RAN Alliance}
%\textcolor{blue}{How organized, who participates, what is standardized}
The O-RAN Alliance was formed by merging the C-RAN Alliance %~\cite{} 
and the xRAN forum%~\cite{}
and leads the open RAN movement that aims to extend the current RAN standards to facilitate open, intelligent, virtualized and fully interoperable next generation RANs. 
Many of its members are also members of the 3GPP. 

 %The O-RAN standards 
Its study items cover the overall O-RAN architecture and is divided into main nine technical work groups (WG):
%The WGs are: 
\begin{itemize}
    \item WG1: Use cases and overall architecture,
    \item WG2: %the %non-real-time RAN intelligent controller
    Non-RT RIC and A1 interface,
    \item WG3: %the %Near-real-time 
    Near-RT RIC and E2 interface,
    \item WG4: Open fronthaul interfaces, 
    \item WG5: Open F1/W1/E1/X2/Xn interface,
    \item WG6: Cloudification and orchestration,
    \item WG7: White-box hardware, 
    \item WG8: stack reference design, and
    \item WG9: open X-haul transport.
\end{itemize}
In addition, there are four O-RAN focus groups (FG) that handle items %topics 
related to the overall mechanism of O-RAN:
\begin{itemize}
    \item FG1: standard development,
    \item FG2: test \& integration,
    \item FG3: open source, and
    \item FG4: security. 
\end{itemize}

Figure~\ref{fig:ORANStnds} illustrates the WGs and FGs defined by the O-RAN Alliance along with the main contributions of each group. The working groups meet regularly and updated specifications are published and made accessible to the community every three months.


% %\subsubsection{Telecom Infrastructure Project (TIP)}
% \hl{Did TIP take off or is it phasing out? If still popular, let's keep it here.} TIP was intially formed by Facebook with a focus on enabling access for all and is currently headed by Vodafone~\cite{}. Unlike the O-RAN Alliance, which mainly concerns itself with an open and interoperable RAN, TIP has many project groups that span a diverse set of wireless communication systems. The project groups are categorized into three main groups which include many sub-groups within them:
% \begin{itemize}
%     \item Product project groups : Focuses on identification of areas in need of innovation. It is divided into three network areas that collectively make up an end-to-end network viz,
%     \begin{itemize}
%         \item Access Projects : RAN Initiatives, Open Cellular and OpenRAN - TIP 
%     \end{itemize}
    
%     \item Solution Project groups
%     \item Software Project groups
% \end{itemize}
% While the O-RAN Alliance heavily focuses on 4G and 5G, TIP 
% \begin{itemize}
%      \item WG1: Use Cases and Overall Architecture Workgroup
%      \item WG2: The Non-real-time RAN Intelligent Controller and A1 Interface Workgroup
%      \item WG3: The Near-real-time RIC and E2 Interface Workgroup
%      \item WG4: The Open Fronthaul Interfaces Workgroup
%      \item WG5: The Open F1/W1/E1/X2/Xn Interface Workgroup
%      \item WG9: Open X-haul Transport Workgroup
%      \item TIFG: Test & Integration Focus Group 
     
%  \end{itemize}

 
%O-RAN Alliance described in Work Grope 1 (WG1) specifications different use cases that leverage the O-RAN architecture and demonstrate its unique benefits to optimize a RAN function and update policies based on performance measurement. some of these used cases deploy one of the aforementioned ML deployment scenario in the O-RAN architecture. 


\subsection{Software} \label{software}
\subsubsection{O-RAN Software Community}
The O-RAN Alliance together with the Linux Foundation officially launched the O-RAN software community (OSC) in April 2019 for the realization of O-RAN components and systems via open-source software. The first code release of the OSC was the Amber release in December 2019. It was been developed by 60 developers across 10 companies and provides initial implementation of the near-RT RIC, O1 interface, and the protocol stack. In June 2020, the Bronze release was the result of 80 contributors from 15 companies. The Bronze contributions focused on the development of the O-DU, O-CU, O1 and A1 interfaces. The Cherry release was presented in December 2020 involving of 60 developers from 10 companies. The Cherry release advances the O1 and A1 interfaces implementations and introduces the E2 interface with end-to-end integration and focus on the SMO components for management and self-organization. The %most recent release, called 
Dawn became available in July 2021 and provides evolved A1, E2, and O1 interfaces with more advanced xApps for near-RT RIC, non-RT RIC use cases and O-DU specifications. A new R1 interface between rapps and SMO/non-RT RIC services was also introduced. Figure.~\ref{fig:ORANStnds} shows the O-RAN software development timeline. % starting from the launching up to the expected E release.

\subsubsection{ONF SD-RAN}
The Open Networking Foundation's software-defined RAN (SD-RAN) project engages in a parallel open source development effort that aims to integrate the 3GPP compliant RAN with the O-RAN RIC and its interfaces along with a few exemplar xApps. The first release of SD-RAN came out in Januray 2021 with support for a near-real time RIC based on ONF's $\mu$ONOS and Aether(VIM) platforms. Open Air Interface 5G~\cite{} enhanced with O-RAN compliant protocols and interfaces is employed to undertake O-DU and O-CU functionalities.  An SDK, portable across different near-RT RIC platforms for the xApp development has also been released. This means that the SDK can also be used in OSC's system. SD-RAN's vision is to expand the E2 interface to allow for scheduler control and implement use cases related to network slicing, handover and load balancing. 

While the SD-RAN uses OAI-5G and potentially provides hardware compatibility, it is designed as a production grade software directed at companies developing intelligent xApps. Therefore SD-RAN's offerings are protected by a member only software license The software framework developed by the OSC implements the control stack and does not support hardware enabled RAN systems yet. Simulated environments such as the O-DU/O-CU code base ~\cite{} and the Viavi RAN simulator~\cite{} serve as options to test and validate the working of the O-RAN system but fall short in terms of measuring the performance in a realistic wireless environment. This served as an inspiration for various independent working groups to develop a hardware compliant Open RAN ecosystem to fully enable design, analysis and testing of solutions in a real-world setting. 
% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/ORAN/ORAN_SW.pdf}
% %\vspace{-70 pt}
% \caption{O-RAN software development timeline.}
% \label{fig:ORANSW}
% \vspace{-3mm}
% \end{figure}


\subsection{Testbeds}
%\begin{itemize}[leftmargin=+9.4pt]
%\item
  

The Platforms for Advanced Wireless Research (PAWR) is a public-private partnership program that supports the develops and maintains five large-scale wireless testbeds, four in realistic outdoor environments and one large-scale programmable RF emulator. It is a National Science Foundation (NSF) initiative. Several PAWR platforms currently work on O-RAN implementations, discussed in continuation.

%\textbf{POWDER:} 
The Platform for Open Wireless Data-driven Experimental Research (POWDER)~\cite{breen2021powder} is a city scale, remotely accessible, end-to-end software defined platform that supports mobile and wireless research. It is deployed in Salt Lake City, Utah. %POWDER has so far deployed over a dozen fixed and approximately fifty mobile programmable radio nodes over an area of 14 square kilometers, covering a variety of distinct environments such as urban, moderate density and residential environments. Experiments over a range of heterogeneous wireless technologies including massive MIMO, 5G, RAN are supported. 
The testbed is equipped with cutting edge software-defined radios (SDRs), commercial off-the-shelf (COTS) equipment and computing resources at both the edge and cloud to support low latency interactions. An experimenter %also allows an experimenter to
can instantiate a series of profiles---a set of experiment environments for popular 4G/5G software stacks, such as srsRAN and OpenAirInterface%(OAI)
, and the Open Network Automation Platform (ONAP) for network control and orchestration. An O-RAN capable profile %with  capabilities was added. It
implements the communication between the near-real time RIC and the RAN node simulated by srsRAN. An xApp featuring basic RAN slicing was also developed to demonstrate how a RAN node can be controlled by the near-RT RIC based on inputs from a \hl{What is this and is it too much detail?}REST server~\cite{Johnson21NexRAN}. 
%to   Some of the "sister" projects of POWDER 

%\textbf{COSMOS}: 
The Cloud-Enhanced Open Software Defined Mobile Wireless Testbed for City-Scale Deployment (COSMOS)~\cite{raychaudhuri2020challenge} is based in New York City. % covering 1 square mile of densely populated neighborhood in West Harlem, New York. 
The focus of COSMOS is on ultra high bandwidth and low-latency communications by employing mmWave and dynamic optical switching technologies and coupling it with edge computing.
COSMOS includes the Open-Access Research Testbed for Next-Generation Wireless Networks (ORBIT)~\cite{} which is compatible with open RAN solutions and served as the Open Test and Integration Center to demonstrate multi-vendor interoperability during the O-RAN plugfest~\cite{}.

% AERPAW (focusing on aerial communication).... 

%\textbf{COLOSSEUM:}
The Colosseum testbed is %one of the world's most powerful full stack
an SDR-based wireless network emulator~\cite{} %based in Burlington, MA at 
that was developed by DARPA and is now maintained by Northeastern University. % Innovation campus. 
%The testbed is a specialized datacenter with up to 900TB of storage, 171 servers, 320 FPGAs and a total of 25.6 GHz of instantaneous bandwidth. 
It includes 256 programmable SDRs (USRP X310s) out of which 128 are dedicated to a massive channel emulator. % (MCHEM) which can emulate almost any real world scenario such as open fields, dense urban cities, deserts, shopping malls etc. %The rest of the 128 nodes are available to experimenters. The MCHEM can emulate fading, multipath for upto 256x256 independently customizable channels. Additionally, the testbed supports cellular networks (4G, 5G), IoT networks, edge computing and cloud based RAN research. 
Several applications are preconfigured by Colosseum and can be instantiated by experimenters in the form of %ready to use 
LXC containers, which can also be customized by users. %The containers can also be customizable by users to implement their own radio codes. The platform also allows implementation and testing of machine learning algorithms for various wireless techniques including spectrum sharing, dynamic spectrum access (DSA) and optimized routing. ML algorithms can be tested by collecting RF data at a rate of 52 TB/s from heterogeneous wireless networks. \hl{Can we elaborate more on O-RAN on Colosseum, and shorten the rest?} 
Recently, open-source RAN solutions were made available with the inclusion of the %O-RAN 
near-RT RIC interfaced with srsLTE~\cite{bonati2020intelligence}. %Colosseum was initially used in DARPA's Spectrum Collaboration Challenge (SC2) until the finals in 2019 and will be available to researchers through NSFs PAWR program henceforth. The testbed is accessible as a cloud based platform where users can reserve resources and schedule experiments manually or configure it as a batch job. 

% {latest PAWR testbed ...}
%\item 
%{\textbf{COLLOSEUM Testbed:}}

%\textcolor{blue}{Briefly comparison of these resources and their capabilities}
 
\subsection{OAIC}
%\textbf{Open Artificial Intelligence Cellular (OAIC):} 
%\hl{Vuk will revise} 
Open Artificial Intelligence Cellular (OAIC) is a large-scale community research infrastructure project that focuses on developing a 6G research framework. It implements and extends the O-RAN framework and interfaces, develops AI controllers, and an AI controllers/O-RAN network testing framework for use with SDR testbeds. It closes the gap between testbed hardware and 5G protocol software development and deployment to enable AI-controlled 5G and 6G research. %and maintenance and community SDR research testbed, such as the PAWR platforms. 
%... a mobile community research testbed infrastructure based in \hl{.....} 
OAIC aims to supplement open SDR platforms and community testbeds with AI-enhanced, O-RAN compliant wireless network functions and controllers to enable research on next generation RANs and advance the %O-RAN 
specifications. 
OAIC also develop the tools and procedures for designing and testing AI-enhanced wireless networks in controlled and production-like environments. %and It is a platform that enables designing and testing AI-driven 6G RAN use cases. The testbed consists of multiple programmable SDRs (B210s and N300s) and servers capable of simulating LTE/5G systems. Recently, the testbed included O-RAN capabalities where the communication between the near-real time RIC and the RAN node, using srsLTE 
%was established. 
Using servers, COTS SDR hardware, and exclusively open-source software, the OAIC team implemented the interfaces between the near-RT RIC and the software-defined LTE base station (srsRAN) and developed a resource allocation xApp %has been developed where the xApp 
which makes decisions on the number of physical resource blocks (PRBs) that have to be allocated to SDR UEs transmitting on both uplink and downlink in a controlled %n SDR LTE 
testbed environment. 
%\end{itemize}



==> include/testbeds.tex <==
\subsection{O-RAN Software Community}
The O-RAN Alliance~\cite{openranalliance} has teamed up with the Linux foundation and has established the O-RAN Software Community (OSC)~\cite{oransoftwarecommunity} to develop open source software compliant with O-RAN specifications~\cite{}. Led by a consortium of major operators and vendors featuring the likes of AT&T, Nokia, Intel, Radisys, 3 releases viz., “amber”, “bronze”, “cherry” have been published. 

% The RIC deployment follows the cloud-based architecture and is implemented on COTS hardware. The near-RT RIC installed on VM has containers for each of its components. The docker containers need to be loaded with the respective images built from the provided source code. Once that is done, the built images need to be hosted on a server from where they can be pulled. Another simpler approach would be to directly pull the docker images from the nexus server hosted by OSC. 

\subsection{ONAP Implementation}
ONAP is an NFV framework developed as a project of the Linux Foundation and major telecom operators such as AT&T, China Mobile, Vodafone, etc. ONAP is deployed in several commercial cellular networks, and vendors like Ericsson, Nokia, Huawei and ZTE, among others, provide ONAP support and integration in their products. Therefore, ONAP represents one of the most advanced software-based solutions for commercial cellular networks, actively maintained and developed to meet production-level quality standards and satisfy new emerging requirements.
ONAP handles the design, creation, and life cycle management of a variety of network services. Network operators can use ONAP to orchestrate the physical and virtual infrastructure
deployed in their networks, in a vendor-agnostic way. In addition to common NFV orchestrator functionalities (e.g., automated policy-driven management of the virtualization infrastructure and of the network services), ONAP provides a design framework to model network applications and services as well as a framework for data analytics to monitor the services for healing and scaling. Additionally, ONAP provides a number of reference designs, i.e., blueprints. 
% These can be used to deploy the ONAP architecture, depicted at a highlevel in Figure 12, in specific markets or for specialized use cases (i.e., 5G networks or Voice over LTE deployments). They
have been tested in combination with their typical hardware configurations.
The main components of 

\subsection{PAWR Testbeds} 
The Platform for Open Wireless Data-driven Experimental Research (POWDER)~\cite{breen2021powder} is a city scale, remotely accessible, end-to-end software defined platform that supports mobile and wireless research currently deployed in Salt Lake City, Utah. Developed as a part of the National Science Foundation (NSF) Platforms for Advanced Wireless Research Programs (PAWR). POWDER has deployed over a dozen fixed and approximately fifty mobile programmable radio nodes over an area of 14sq.km. covering a variety of distinct environments such as urban, moderate density and residential environments. Experiments over a range of heterogeneous wireless technologies including massive MIMO, 5G, RAN is supported. The testbed is equipped with cutting edge SDRs, COTS equipment and computing resources at both the edge and cloud to support low latency interactions. The platform also allows an experimenter to instantiate a series of "profiles" - set of experiment environments for popular 4G/5G software stacks such as srsRAN, OpenAirInterface, ONAP for network control and orchestration. Recently a profile with O-RAN capabilities was added  to   Some of the "sister" projects of POWDER include  COSMOS~\cite{raychaudhuri2020challenge} (focusing on mmWave technology) and AERPAW (focusing on aerial communication). COSMOS includes the Open-Access Research Testbed
for Next-Generation Wireless Networks (ORBIT) ~\cite{} which is compatible with open RAN solutions and served as the Open Test and Integration Center to demonstrate multi-vendor interoperability during the O-RAN plugfest~\cite{}.

\subsection{COLLOSEUM Testbed}
\textcolor{blue}{Comparison of these resources and their capabilities}

